A Bound for the Locating Chromatic Numbers of Trees

Let $f$ be a proper $k$-coloring of a connected graph $G$ and $\Pi=(V_1,V_2,\ldots,V_k)$ be an ordered partition of $V(G)$ into the resulting color classes. For a vertex $v$ of $G$, the color code of $v$ with respect to $\Pi$ is defined to be the ordered $k$-tuple $c_{{}_\Pi}(v)=(d(v,V_1),d(v,V_2),\ldots,d(v,V_k)),$ where $d(v,V_i)=\min\{d(v,x): x\in V_i\}, 1\leq i\leq k$. If distinct vertices have distinct color codes, then $f$ is called a locating coloring. The minimum number of colors needed in a locating coloring of $G$ is the locating chromatic number of $G$, denoted by $\Cchi_{{}_L}(G)$. In this paper, we study the locating chromatic numbers of trees. We provide a counter example to a theorem of Gary Chartrand et al. [G. Chartrand, D. Erwin, M.A. Henning, P.J. Slater, P. Zhang, The locating-chromatic number of a graph, Bull. Inst. Combin. Appl. 36 (2002) 89-101] about the locating chromatic numbers of trees. Also, we offer a new bound for the locating chromatic number of trees. Then, by constructing a special family of trees, we show that this bound is best possible.

==> README <==

                               The xargs package

            Defining commands with many optional arguments made easy

               Manuel P\'egouri\'e-Gonnard <mpg@math.jussieu.fr>


Presentation
------------

Defining commands with an optional argument is easy in LaTeXe. There is,
however, two limitations: only one argument can be optional and it must
be the first one. The xargs package provide extended variants of
\newcommand & friends, for which these limitations no longer hold. It
allows to control what happens with many consecutive optional arguments.
It also provide a way of making the definition global.

Some features of xargs are similar to those provided by the experimental
`xparse' package, which also allows more flexible argument syntaxes,
though the approach and syntax are different.  However, xargs is not
experimental, so I hope it can be useful while waiting for a stable
LaTeX3 release.

Contents
--------

xargs.sty:      the package itself
xargs.pdf:      the (English) documentation and documented code
xargs-fr.pdf:   the French documentation

xargs.dtx:      source for both documentations and package

Version info
------------

2007-10-20  v1.0    First release
2008-03-08  v1.09   Added the usedefault and addprefix keys, not
                    documented yet...
2008-03-22  v1.1    Updated the documentation and fixed a bug in
                    \DeclareRobustCommandx, introduced in v1.09.

License
-------

This material is subject to the LaTeX Project Public License. See
http://www.ctan.org/tex-archive/help/Catalogue/licenses.lppl.html for the
details of that license.


